Formal verification of Zagier's one-sentence proof

We comment on two formal proofs of Fermat's sum of two squares theorem, written using the Mathematical Components libraries of the Coq proof assistant. The first one follows Zagier's celebrated one-sentence proof; the second follows David Christopher's more recent proof relying on partition-theoretic arguments. Both formal proofs rely on a general property of involutions of finite sets, of independent interest. The proof technique consists for the most part of automating recurrent tasks (such as case distinctions and computations on natural numbers) via ad hoc tactics. With the same method, we also provide a formal proof of another classical result on primes of the form $a^2 + 2 b^2$.

==> defManSSR.tex <==
%=======================================================================
% A listing mode for ssr Gallina (Assia Mahboubi 2007)
% Used by G. Dubach and F. Mühlböck with authorisation from the original author, 2021
\lstdefinelanguage{SSR} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside, outside},

% Gallina
morekeywords=[2]{forall, exists, exists2, fun, fix, cofix, struct,
      match, with, end, as, 
      %in ,
      return, let, if, is, then, else,
      for, nosimpl},
% 'of' is removed from this list as it occurs in comments.

% Sorts
morekeywords=[3]{Type, Prop, choiceType,fset, fsetval},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{
         pose, set, move, case, elim, apply, clear,
            hnf, intro, intros, generalize, rename, pattern, after,
            destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, ring, field,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr, vm_compute,
         symmetry, transitivity, auto, split, left, right,
         autorewrite, lia, intlia},

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},

% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
 literate=
%        {|in}{$\in $ }2
%        {#|`}{|}1
%        {`\backslash`}{$\backslash$}2 does not work...
        {->}{{$\rightarrow\ $}}2
%       {->}{{\tt ->}}3
%	{<-}{{$\leftarrow\,$}}2
%       {<-}{{\tt <-}}2
%       {>->}{{$\mapsto$}}3
        {<}{{$<\;\;$}}1
        {<=}{{$\leq\;\;$}}1
        {>=}{{$\geq\;\;$}}1
%       {<>}{{$\neq$}}1
        {/\\}{{$\wedge\;\;$}}2
        {\\/}{{$\vee\;\;$}}2
        {^~}{{\textvisiblespace$\;\;$}}2
        {~~}{{$\lnot\;\;$}}2
%       {<->}{{$\leftrightarrow\;$}}3
%       {<=>}{{$\Leftrightarrow\;$}}3
%       {:nat}{{$~\in\mathbb{N}$}}3
%	{fforall\ }{{$\forall_f\,$}}1
	{forall\ }{{$\forall\ \!$}}1
	{exists\ }{{$\exists\ \!$}}1
        {MAPLE}{{\raisebox{-0.8cm}[0cm][0cm]{\hspace{18mm}\includegraphics[width=1cm]{maple}}}}1
	{^2}{{$^2$}}1
	{^3}{{$^3$}}1
	{^4}{{$^4$}}1
	{^5}{{$^5$}}1
	{^6}{{$^6$}}1
%       {negb}{{$\neg$}}1
%       {spp}{{:*:\,}}1
%       {~}{{$\sim$}}1
%       {\\in}{{$\in\;$}}1
%       {/\\}{$\land\,$}1
%       {:*:}{{$*$}}2
%	{=>}{{$\,\Rightarrow\ $}}1
%       {=>}{{\tt =>}}2
%       {:=}{{{\tt:=}\,\,}}2
%       {==}{{$\equiv$}\,}2
        {!=}{{$\neq$}\ }2
        {_cf0}{{$_{{0}}$}}1
        {_cf1}{{$_{{1}}$}}1
        {_cf2}{{$_{{2}}$}}1
        {_cf0_0}{{$_{{00}}$}}1
%        {_cf0}{{$_{\mbox{cf}_{0}}$}}1
%        {_cf1}{{$_{\mbox{cf}_{1}}$}}1
%        {_cf2}{{$_{\mbox{cf}_{2}}$}}1
%        {_cf0_0}{{$_{\mbox{cf}_{00}}$}}1
%       {^-1}{{$^{-1}$}}1
%       {elt'}{elt'}1
%       {=}{{\tt=}\,\,}2
%       {+}{{\tt+}\,\,}2
,

% Comments delimiters, we do turn this off for the manual
%comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",

% Size of tabulations
tabsize=3,

% Enables ASCII chars 128 to 255
extendedchars=true,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily\footnotesize,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]fullflexible,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{dkviolet}},

% Style for gallina keywords
keywordstyle=[2]{\ttfamily\color{dkgreen}},

% Style for sorts keywords
keywordstyle=[3]{\ttfamily\color{lightgreen}},

% Style for tactics keywords
keywordstyle=[4]{\ttfamily\color{dkblue}},

% Style for terminators keywords
keywordstyle=[5]{\ttfamily\color{red}},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
%commentstyle=\rmfamily,

}

